A Dictionary-based Approach to Racism Detection in Dutch Social Media

We present a dictionary-based approach to racism detection in Dutch social media comments, which were retrieved from two public Belgian social media sites likely to attract racist reactions. These comments were labeled as racist or non-racist by multiple annotators. For our approach, three discourse dictionaries were created: first, we created a dictionary by retrieving possibly racist and more neutral terms from the training data, and then augmenting these with more general words to remove some bias. A second dictionary was created through automatic expansion using a \texttt{word2vec} model trained on a large corpus of general Dutch text. Finally, a third dictionary was created by manually filtering out incorrect expansions. We trained multiple Support Vector Machines, using the distribution of words over the different categories in the dictionaries as features. The best-performing model used the manually cleaned dictionary and obtained an F-score of 0.46 for the racist class on a test set consisting of unseen Dutch comments, retrieved from the same sites used for the training set. The automated expansion of the dictionary only slightly boosted the model's performance, and this increase in performance was not statistically significant. The fact that the coverage of the expanded dictionaries did increase indicates that the words that were automatically added did occur in the corpus, but were not able to meaningfully impact performance. The dictionaries, code, and the procedure for requesting the corpus are available at: https://github.com/clips/hades

==> figure_CV_vs_test.tex <==
\begin{figure}
\begin{tikzpicture}[scale=0.85]
    \begin{axis}[
        ymin = 0,
        ymax = 1,
        width  = 0.95*\textwidth,
        height = 8cm,
        major x tick style = transparent,
        ybar,
        bar width=20pt,
        x={2*14+60pt},
        enlarge x limits={abs=14pt+30pt},
        %% LH bovenstaande twee regels toegevoegd om mooie spacing te hebben
        %% http://tex.stackexchange.com/questions/120026/pgfplots-dollar-sign-in-node-adjust-space-between-bars
        ymajorgrids = true,
        ylabel = {Score},
        symbolic x coords={train,test},
        xtick = data,
        ytick={0,0.1,...,1},
        %% LH bovenstaande lijn verwijderen om terug schaling per 0.2 te hebben
        scaled y ticks = false,
        legend style={at={(0.5,-0.15)},
        anchor=north,legend columns=-1},
    ]
    
        \addplot[style={bblue,fill=bblue,mark=none}]
        coordinates {(train, 0.85) (test, 0.73)};
            
        \addplot[style={rred,fill=rred,mark=none}]
        coordinates {(train, 0.80) (test, 0.73)};
        
        \addplot[style={ggreen,fill=ggreen,mark=none}]
        coordinates {(train, 0.71) (test, 0.66)};



        \legend{precision, recall, F1}
    \end{axis}
\end{tikzpicture}
\caption{Average of precision, recall, and F1 on train and test data}
\end{figure}

==> figure_prf_per_class.tex <==
\begin{figure}
\begin{tikzpicture}[scale=0.85]
    \begin{axis}[
        ymin = 0,
        ymax = 1,
        width  = 0.95*\textwidth,
        height = 8cm,
        major x tick style = transparent,
        ybar,
        bar width=20pt,
        x={2*14pt+60pt},
        enlarge x limits={abs=14pt+30pt},
        ymajorgrids = true,
        ylabel = {Score},
        symbolic x coords={racist,non-racist},
        xtick = data,
        ytick={0,0.1,...,1},
        scaled y ticks = false,
        legend style={at={(0.5,-0.15)},
        anchor=north,legend columns=-1},
    ]
    
        \addplot[style={bblue,fill=bblue,mark=none}]
        coordinates {(non-racist, 0.82) (racist, 0.50)};
            
        \addplot[style={rred,fill=rred,mark=none}]
        coordinates {(non-racist, 0.81) (racist, 0.51)};
        
        \addplot[style={ggreen,fill=ggreen,mark=none}]
        coordinates {(non-racist, 0.82) (racist, 0.51)};


        \legend{precision, recall, F1}
    \end{axis}
\end{tikzpicture}
\caption{Precision, recall, and F1 for each class (test set)}
\end{figure}

==> figure_recall_vs_freq.tex <==
\begin{figure}
\begin{tikzpicture}[scale=0.85]
    \begin{axis}[
        ymin = 0,
        ymax = 1,
        width  = 0.95*\textwidth,
        height = 8cm,
        major x tick style = transparent,
        ybar,
        bar width=20pt,
        x={2*14pt+40pt},
        enlarge x limits={abs=14pt+20pt},
        ymajorgrids = true,
        ylabel = {Score},
        symbolic x coords={racist,non-racist},
        xtick = data,
        ytick={0,0.1,...,1},
        scaled y ticks = false,
        legend style={at={(0.5,-0.15)},
        anchor=north,legend columns=-1},
    ]
    
        \addplot[style={bblue,fill=bblue,mark=none}]
        coordinates {(non-racist, 0.81) (racist, 0.51)};
            
        \addplot[style={rred,fill=rred,mark=none}]
        coordinates {(non-racist, 0.82) (racist, 0.18)};
        
        \legend{recall, corpus frequency}
    \end{axis}
\end{tikzpicture}
\caption{Recall vs. corpus frequency for each class}
\end{figure}
